Towards a Flexible and High-Fidelity Approach to Distributed DNN Training Emulation

We propose NeuronaBox, a flexible, user-friendly, and high-fidelity approach to emulate DNN training workloads. We argue that to accurately observe performance, it is possible to execute the training workload on a subset of real nodes and emulate the networked execution environment along with the collective communication operations. Initial results from a proof-of-concept implementation show that NeuronaBox replicates the behavior of actual systems with high accuracy, with an error margin of less than 1% between the emulated measurements and the real system.

==> sections/abstract.tex <==
%The groundbreaking advances that Deep Neural Networks (DNNs) have achieved in various application domains are accompanied by a significant underutilization of compute resources in scale-out data center networks and AI clusters. 
%Efficient system configuration is essential to optimizing cluster utilization and addressing the escalating costs of training large models. However, the prohibitive time and cost implications of exploring configurations on real hardware emphasize the need for a fast, cost-effective, and high-fidelity approach to testing cluster configurations prior to deployment for DNN training. Existing simulation-based methods, while promising, often suffer from technical complexity, limited adaptability, or limited accessibility. To mitigate these limitations, 


We propose \sys, a flexible, user-friendly, and high-fidelity approach to emulate DNN training workloads. We argue that to accurately observe performance, it is possible to execute the training workload on a subset of real nodes and emulate the networked execution environment along with the collective communication operations. Initial results from a proof-of-concept implementation show that \sys replicates the behavior of actual systems with high accuracy, with an error margin of less than 1\% between the emulated measurements and the real system.





==> sections/background.tex <==
The Data Parallel (DP) distributed training paradigm is typically adopted when the size of a DNN model fits within the memory of a single compute workers~\cite{xing2015petuum}. Under this paradigm, the model is replicated across multiple compute workers, with the training data partitioned among these workers. Weight aggregation among workers occurs at periodic intervals during training, facilitated by collective communication primitives. Conversely, when the model exceeds the memory capacity of a single compute worker, various distributed training methodologies can be employed, including Pipeline Parallel (PP)~\cite{huang2019gpipe}, Tensor Parallel (TP)~\cite{shoeybi2020megatronlm}, and Fully Sharded Data Parallel (FSDP)~\cite{zhao2023pytorch} approaches. In all of these methodologies, the model is partitioned among multiple compute workers, with intermediate computation results exchanged, alongside weight aggregation akin to DP.

All of the distributed training strategies described above rely on collective communication operations to synchronize intermediate results across several processing units during training. Table \ref{table:coll} outlines the specific collective operations employed by each strategy~\cite{rajbhandari2020zero, shoeybi2020megatronlm}.

\begin{table}[htb]
\centering
\begin{tabular}{ |c|c|c|c| } 
\hline
Data & Inter Op & Intra Op & Fully-Sharded  \\
\hline
allreduce & allreduce & allreduce & reduce-scatter \\ 
 & p2p & allgather & allgather \\ 
\hline
\end{tabular}
\caption{Collective Operations Used In Different Parallel Strategies. We only list operations used at least once per iteration, those only used in initialization(i.e. broadcast) are not shown}
\label{table:coll}
\end{table}

These collective operations perform all necessary synchronizations implicitly, so no additional control logic is required beyond the initial launch of the training script. This makes the collective communication layer a valuable channel for studying the communication behavior inherent in different distributed training strategies and how it affects the overall training performance.

% An example of a four node training using distributed data parallel will be used to illustrate the idea, and more complex scenario like non-uniform and async workload will be discussed later.

% \begin{algorithm}
% \caption{Naive Distributed Data Parallel}\label{alg:cl}
% \begin{algorithmic}
% \Procedure{averagegradient}{$model, myrank, nranks$}
%   \State $my\_grad \gets model.params.gradient()$ 
%   \State $new\_grad \gets allreduce(my\_gradient, mrank, nranks)$ 
%   \Return $new\_grad$
% \EndProcedure
% \State $model \gets DDPWrapper(model, loss)$
% \While{training}
% \State $model.forward()$
% \State $model.backward()$
% \State $gradient \gets average\_gradient(model, myrank, nranks)$
% \State $model.update(gradient)$
% \EndWhile

% \end{algorithmic}
% \end{algorithm}

% We can see that there is no other network communication rather that in $average\_gradient$, which fires $allreduce$. If we can mock the data that $N_0$ needs to send and receive in each $allreduce$ call, we are able to mock the whole training process.


%\subsection{Resource Utilization}
%Distributed DNN training relies on the robust infrastructure of large-scale clusters and dedicated data center networks. However, despite the substantial computational resources and networking infrastructure available, the full computational capacity of these clusters remains underutilized, with utilization rates typically ranging between 5–20\% during the training of large models~\cite{ardalani2022deepflow}. In this situation, an efficient configuration is essential not only to optimize DNN training performance but also to maximize the utilization of cluster resources. However, the process of testing all potential system configurations on actual cluster infrastructure is prohibitively expensive, time-consuming, and impractical for many organizations and institutions. This phenomenon underscores the need for a fast, cost-effective, and high-fidelity approach to testing cluster configurations prior to deployment for DNN training.


\smartparagraph{Simulation.}
%\subsection{Simulation}
\label{sec:background:simulation}
Several simulators have been proposed to investigate the performance of different system configurations in distributed training\cite{rashidi2022themis, won2023astra, bang2023vtrain, esposito2022dts}. Although simulation-based approaches provide valuable insights into the performance of DDL training clusters, they have several drawbacks that limit their effectiveness. First, simulators often require significant technical expertise to configure and operate, making them inaccessible to researchers and organizations without specialized knowledge. In addition, these simulators lack the flexibility to adapt to evolving distributed training paradigms and hardware architectures, resulting in inaccurate performance predictions. For example, to the best of our knowledge, none of the existing simulators support FSDP. Furthermore, simulators typically rely on models of system behavior that, while very effective, may not fully capture the complexity of actual execution environments. These limitations undermine the applicability of simulation-based approaches, and emphasize the need for complementary and/or alternative methods.

Some other works~\cite {stanic2023languini, hestness2017deep} use some linear models to estimate the training time of DNNs, based on the available compute resources in FLOPs.A limitation of this approach is that the assumption about the available FLOPs does not take into account different system characteristics and configurations (e.g., bandwidth, topology, distributed training strategy, etc.) that could affect the available compute resources.

\smartparagraph{Emulation.}
%\subsection{Emulation}
\label{sec:background:emulator}
While simulators focus on predicting system behavior based on predefined models and assumptions, emulators offer a more dynamic and flexible approach. Emulators can directly replicate the behavior of distributed training jobs, enabling a more accurate representation of real-world scenarios. Specifically, unlike simulators, which are based only on performance models and profiled metrics, emulators recreate the actual behavior of the underlying hardware with high fidelity, allowing them to more accurately predict the behavior of the system under evaluation. Furthermore, Emulators can serve as a complementary tool to simulators by addressing certain limitations and providing unique insights into the performance optimization of training clusters. 

%\banruo{Though widely used in networking research, to the best of our knowledge, emulator has not been adopted in distributed training research. One reason is because lacks scalability, since aggregate bandwidth grows as cluster becomes larger. We address this problem by exploiting the scale-free operations.}



%By emulating the communication patterns of DDL frameworks, we can gain valuable insights into the performance characteristics of distributed training tasks and identify optimization opportunities to enhance overall system efficiency. With emulators, changes in abstraction or implementation details can be more easily supported, largely without modification.





==> sections/conclusion.tex <==
We proposed a novel approach for estimating time-per-iteration in distributed DNN training, focusing on executing only a part of the model along with collective communication operations. To substantiate our proposal, we designed the \sys emulator and implement a proof-of-concept system. Through extensive experimentation, we demonstrated in a two-node setup that \sys achieves high accuracy in predicting training time across a variety of DNN models, with an error margin of less than 1\% compared to actual training runs. Finally, we encourage further research in this direction, recognizing that many questions remain to be explored.

%Specifically, we observe that most distributed training strategies aim to distribute the workload evenly among compute workers to ensure that computations are completed at approximately the same time, and synchronisation can subsequently begin through collective communication. Based on this observation, we argue that to accurately predict the training time per iteration, it is sufficient to emulate the computation on only one(part) of the compute nodes along with the collective communication operations. This approach offers inherent flexibility to support diverse parallelization strategies, ease of use, fidelity to actual training runs, and resource efficiency.

==> sections/design.tex <==
Our goal is to enable any subset $\nbReal$ of nodes in a distributed DNN training job to execute the workload as if it were running on the entire set of nodes and resources. We propose to achieve this goal by emulating the interactions between $\nbReal$ and its networked environment $\nbEnv$, which in a sense can be viewed as a virtualization of the remaining job's nodes.
We argue that, under certain assumptions (detailed below), by observing the performance of $\nbReal$, we can analyze and extrapolate the behavior for an entire job with high fidelity.

In our design, we adhere to two driving principles:

% \mcnote{scratch}
% Our approach is to emulate the networked environment around a real node. In other words, we virtualize the remaining nodes and emulates the interactions between the real node and the virtualized nodes. We posit this approach allows us to accurately predict the behavior of the entire workload by observing the behavior of a single node.

% An important question is how to emulate the interactions between the real node and the virtualized nodes. We propose to focus on the collective communication layer, which bridges the gap between network packets and computational graph operators. This level of granularity avoids the complexity of packet-level emulation and still allows us to capture network-level performance behavior.

% What assumptions do we make? Are there observations about common traits of distributed training jobs that we can leverage to justify the assumptions?

% Uniformity of resources: We assume that all nodes in the cluster have identical hardware and topology. This assumption is common in distributed training scenarios, where the goal is to achieve a balanced workload distribution across all nodes. This assumption allows us to treat a single node as a representative of the entire cluster.

% At which level do we emulate? We could intercept at the level of PyTorch, CUDA, or even the network stack. We choose to intercept at the collective communication layer because ...

% We assume that $\nbReal$ has sufficient capacity to host a copy of the model. We believe this is not a strong assumption because it is common to use model or tensor parallelism within a node.

% \subsection{Overview}

% The emulation approach proposed in this work is based on the observation that a single node $N_0$ (consisting of one or more compute workers) in the training job uses collective operations to interact with all other nodes or the ``outside world.'' Specifically, the completion time of a training iteration in a distributed cluster is composed of the time required for the slowest worker machine to complete its computation and the time for collective communication (for synchronizing gradients and weights). Assuming that there are no stragglers and that all nodes have identical behavior, the iteration time can be effectively estimated by measuring the computation time on any node and the collective communication time in the entire training cluster.

%For example, consider a scenario where $\nbReal$ coordinates gradient updates with other nodes in a distributed training task. By accurately measuring the gradient computation time and mimicking the communication patterns between $\nbReal$ and the external nodes, we can effectively simulate the behavior of a distributed training cluster. This approach allows $\nbReal$ to believe it is operating within a cluster environment with multiple nodes, while in reality, these interactions are emulated.
% Suppose there is a cluster running a distributed training workload. The goal of the emulation is to (1) arbitrarily select a node in the cluster; we call it $N_0$. (2) Then we emulate other nodes in the cluster, ``the outside world'' of $N_0$. We intercept and emulate any interaction between $N_0$ and the outside world. (3) The result is that we make $N_0$ believe that it is running the job in the cluster, when in reality only $N_0$ itself is doing work. 

% We argue that by measuring the performance results on $N_0$, we can reliably predict the behavior for the entire cluster. Consider a cluster where the role, workload, topology, and hardware of each node are indistinguishable. Due to this symmetry, the performance of a single node is statistically equal to that of the entire cluster. We call this a uniform scenario, and we discuss how to extend our arguments to a non-uniform scenario in Section~\ref{sec:design:non-uniform}. We also adhere to the following principle in the design of the \sys: 

\smartparagraph{1) Ease of use.}
% Our aim is to make the emulator as easy to use as possible. To this end, we ensure that the Emulator's interfaces are consistent with the popular PyTorch interfaces, and users can directly use their PyTorch code without any modification.
The user should be able to use \sys without any modification to their existing code.

\smartparagraph{2) Flexibility and independence of parallelization strategies.}
%As discussed in \ref{sec:background:simulation}, simulation fails to support new parallelization strategy, making it difficult for academia to test our new ideas. Our emulator is designed to seamlessly adapt to any strategy that does not change collective communication level primitives.
\sys should target a level of abstraction that is independent of the specific parallelization strategy.
\sys should be flexible to seamlessly adapt to changes in parallelization strategies, including new ones that may emerge in the future.
%A limitation of existing simulators is that they have baked-in support for specific parallelization strategies, which hinders experimentation.

% the lack of support for newer parallelization strategies, making them unsuitable for scientific investigations as soon as a new strategy appears. Avoiding this shortcoming is central to our design: \sys is able to seamlessly adapt to changes in training strategy, as long as this strategy is based on collective operation.

% \smartparagraph{Balance between accuracy and complexity.}
% We focus on collective communication abstraction, which bridges the gap between network packets and computational graph operators. This level of granularity avoids the complexity of packet-level emulation and still allows us to capture network-level performance behavior.



% We focus on the collective communication layer, which strikes at the balance of granularity in deep learning jobs. This level of granularity enables us to comprehensively capture network behavior, surpassing model-only approaches. Simultaneously, we avoid delving into packet-level emulation, which could prolong emulation time unnecessarily.

\smartparagraph{Workflow and architecture.}
\cref{fig:overview} depicts an overview of our approach.
The high-level workflow of \sys is as follows.
First, the user provides the training script, the job configuration (e.g., world size, nodes in $\nbReal$, HW resources, etc.), and optionally a set of what-if conditions for experimentation (an example is given later).
Second, \sys initializes the emulation environment by synthesizing the network topology and instantiating a communication model that calculates delay times for collective operations within the emulated environment.
Third, the training script is launched (e.g., via \textsf{torchrun}). Meanwhile, desired performance metrics like iteration time and resource utilization are gathered in $\nbReal$. Traces of collective communication (e.g., NCCL traces) can also be collected.

\smartparagraph{Assumptions.}
We assume that nodes have uniform hardware and network configuration.
In practice, it is common to execute distributed training jobs on homogeneous clusters ~\cite{wang2023zero++,osdi22alpa,touvron2023llama,liu2019roberta,lai2023adaembed}. 
We assume that the model fits entirely within $\nbReal$. This assumption is not restrictive, as it is common to use model or tensor parallelism within a node or a shard~\cite{hwang2023tutel,shoeybi2020megatronlm} . 
We expect that these assumption yield a sort of symmetry in the workload distribution across the nodes, which allows us to treat the nodes in $\nbReal$ as a representative sample of the entire nodes.
We discuss how to extend our arguments to a non-uniform scenario in \cref{sec:design:non-uniform}.

Further, we assume that the collective communication layer is the only point of interaction between $\nbReal$ and $\nbEnv$. This assumption is reasonable, as the collective communication layer is the primary interface between the computation and the network stack in distributed training jobs.
Finally, note that we are free to modify the DNN framework and collective communication libraries within the emulator. That is how we are able to implement \sys!

\smartparagraph{Scalability.}
While collective communication is a natural layer to target in our work, the astute reader may now wonder how scalable this approach is.
Scalability is traditionally a challenge in network emulators~\cite{mininet,modelnet}, as emulating a large number of nodes could overload the emulator.
Our key insight is that we are only interested in the interaction between $\nbReal$ and the outside world. And so, the actual communication between the emulated nodes can be skipped.
Instead, only the delay resulting from these communication operations needs to be incorporated into the emulation. As a result, the number of connections as well as the amount of data transfer for \sys are the same as that of $\nbReal$. This observation allow \sys to potentially scale to a large number of nodes. A complete exploration of the scalability of \sys is left for future work.

In the remainder of this section, we detail the design and implementation of our proposed approach, \sys. Since we aim to demonstrate feasibility through a proof-of-concept, we focus on a single real node, denoted by $N_0$. That is, $\nbReal = \{N_0\}$.

\begin{figure}[t!]
  \centering
  {
\includegraphics[width=0.975\linewidth]{images/overview.pdf}
  }
  \caption{Overall workflow and architecture of \sys.}
 % \caption{The overall architecture and workflow of the emulator. Step \ding{172}Inputs are fed into the emulator.
 % Step \ding{173}emulator initializes itself by synthesizing the artificial cluster. Step \ding{174} Training job is launched. Step \ding{175} Topology detection and connection establishment between $\nbReal$ and emulated cluster. Step \ding{176} The actual training step, which includes computation on $\nbReal$ and communication between $\nbReal$ and the cluster. Step \ding{177} The output is measured based on the time elapsed in the previous step}.
  % \todo{Put "(\%)" in the x-axis label.}
  \label{fig:overview}
\end{figure}

\subsection{Initialization} \label{sec:design:init}

Before we describe how \sys behaves during training, we first need to initialize the emulator. This requires setting up the environment, including the network topology and the communication model.

\smartparagraph{Topology detection.}
\label{sec:design:topology}
This step involves establishing the connection between any pair of nodes, and finding the optimal data paths between all node pairs. It is normally bootstrapped by the collective communication library itself. During this process, each node builds up its own local topology graph (how HW accelerators are connected via NVLink, PCIe and NICs), then exchanges its local graph and, together with other nodes, builds the global graph.
In \sys, the emulator fakes the local graph of emulated nodes based on the job configuration input. Then, it emulates multiple end points (the virtualized job nodes) so that nodes in $\nbReal$ can communicate with them (directly via RDMA).



% \banruo{I want to talk about the scalability here since it has been a concern for emulators in the meeting with Wei Bai. I also want to motivate why we need delay calculation ---- because we omit all computation and data transfer, so we need some reliable method to produce the effect that those omitted operation will cast on $\nbReal$}

\smartparagraph{Delay calculation.}
Based on the global topology, \sys calculates the communication and computation delays within the emulated environment. In our design, we provide an interface so that the calculation itself is done within a user-defined add-on plugin. For example, the delay in a ring all-reduce call can be estimated simply by using the classical all-reduce delay model~\cite{thakur2005optimization}, or by using a packet-level simulator.
In the future we seek to leverage the network simulation components of DNN simulators~\cite{ardalani2022deepflow, won2023astra, bang2023vtrain}.
%$t_{one-hop}*N_{hops}$ 
\subsection{Emulation in a Uniform Scenario} \label{sec:design:uniform}

\begin{figure}[t!]
  \centering
{
\includegraphics[trim={0 0.7cm 0 0},width=0.975\linewidth]{images/dag_view.pdf}
\includegraphics[width=0.975\linewidth]{images/merge_dag.pdf}
  }
  \caption{An example DAG for four-node ring all-reduce. The upper left squares shows the net result of all-reduce, where color-coded data from different nodes are reduced and then gathered at each node. The upper right figure shows the dependency DAG for $\nbReal$ ($N_0$). The lower figure shows how we merge the dependency DAG of $N_1, N_2, N_3$ into $\nbEnv$. The cross-node dependencies from $send(x)$ to $recv(x)$ are not shown for clarity sake. We only show the initial 4 steps of all-reduce for simplicity. }
  % Suppose the cluster has four nodes: $a$, $b$, $c$, $d$. Each node holds its own data that is split into four blocks. We use $a_i$ or $a[i]$ to specify the $i^{th}$ block of data that node $a$ holds. The goal of all-reduce is to perform a collective computation (in this case, a sum operation) on the data held across $a$ to $d$, then distribute the result back to each participating node. The net effect is to make the data end up in each node as $a_i+b_i+c_i+d_i$ for each $i$. We only show the initial 4-step ring-all-reduce message.  We omit the dependency from $send(x)$ to $recv (x)$ for the sake of clarity. \textcolor{blue}{We choose node $a$ (blue background) as $\nbReal$ and emulating its outside world: nodes $b$, $c$, $d$ (grey background), the simplified DAG of \sys(orange background) has the same number of nodes and edges of that of node $a$
  \label{fig:dag}
\end{figure}

In general, a collective operation (e.g., ring all-reduce) can be split into a number of messages with dependencies. The emulator must send/receive messages in a way that takes into account both the dependency and the internal protocol of the collective operations library (in our case, NCCL). We first describe how we treat a single collective operation and then generalize to multiple asynchronous collective operations.

\smartparagraph{Single collective operation.}
Recall that we only need to consider the interaction between $\nbReal$ and $\nbEnv$. This means that we can omit the dependencies for communication within $\nbEnv$.
The workflow of a collective operation can be represented as a directed acyclic graph (DAG) where vertices are send or recv tasks and edges are the data dependencies.
Thus, we note that in \sys, this DAG can be greatly simplified. \cref{fig:dag} shows an example for ring all-reduce.\footnote{The all-reduce operation performs reduction on data (i.e., sums) across nodes and stores the result in a buffer at every node. We use different color for data in different worker.} It is worth noting that the DAGs for $\nbReal$ and \sys are isomorphic. As a result, with every message received from $\nbReal$ to $\nbEnv$, we can always determine the correct state in order to generate the next message of the collective operation workflow.

To achieve this, $\nbEnv$ maintains a bitmap of the messages that have been sent to or received from $\nbReal$, and it applies the following two actions ($\nbEnv$ polls these using background threads) that advance the state of the DAG ensuring synchronization correctness:
% In this case, we maintain a bitmap in the emulator to keep track of the messages received from or sent to node $\nbReal$. We define two functions that are polled by the emulator to ensure that the emulator accurately tracks the exchange of messages with node $\nbReal$ during collective operations and maintains synchronization and correctness throughout the emulation process. These functions are:


\noindent 1) \textit{Try Send To $\nbReal$}. A message can be sent if and only if all its predecessors have been sent or received in the DAG. If the next unsent message in the bitmap fulfils this condition, we update the bitmap and send the message.

% Depending on the type of collective operation, there are distinct synchronization points. It must therefore be ensured that the messages are not sent prematurely. When this function is invoked, we first check the bitmap to determine if the next pending message can be transmitted. If this is the case, we update the bitmap and transmit the message.

\noindent 2) \textit{Try Receive From $\nbReal$}. Upon receiving a message from $\nbReal$, $\nbEnv$ checks whether it is the expected message for the current operation. If this is the case, the bitmap of the record is updated; otherwise, an error is reported.

% There is no need to manually send an acknowledgement, as this is handled by the network layer.


\smartparagraph{Multiple async collective operations.}
The design of a single collective operation can easily be extended to support multiple operations by assigning a unique ID to each operation and maintaining its information in a logically centralized controller. We record the mapping of operations to their message bitmaps. We ensure fairness between the individual streams through round-robin polling. Note that the method for single operation is asynchronous by nature, as the functions are polled by background threads. Given that, the synchronization is achieved by busy-waiting. % for the operation to finish.

\subsection{Extension to a Non-uniform Scenario} \label{sec:design:non-uniform}

%In a uniform setting, the computation profile of a single node effectively reflects that of the entire cluster. This is the usually the case across different parallelization strategies~\cite{hwang2023tutel}.
The workload of individual nodes in a training job may not always be balanced. This is the case, for example, when model parallelism fails to achieve a balanced workload distribution, or when there is heterogeneity of hardware and topology. Consequently, emulating the behavior of an arbitrary node subset ($\nbReal$) may not adequately represent the behavior of the entire workload. To overcome this challenge, we propose to classify each node in the job based on the part of the model it contains, e.g., like having different stages in model parallelism. We then ensure that one node in each class is in $\nbReal$. This approach allows us to infer the behavior of the workload by observing the collective behavior of each class of nodes. This approach also solves the heterogeneity of hardware and topology when we classify nodes with different hardware into different classes.

However, we note that this approach requires more resources. Suppose there are $m$ classes; in the basic solution, we need to have one representative real node for each of them. And with $t$ hardware types, we then need $tm$ nodes in $\nbReal$.
We conjecture that it may be possible to reduce the number of nodes in $\nbReal$, say to $k$, by decoupling the emulation between different nodes. Assuming nodes in $\nbReal$ are in different classes, if all the communication is interposed by $\nbEnv$, then we can time-multiplex the class-based workload and assign each node $\frac{m}{k}$ amount of load.
We leave the exploration of these techniques for future work.

% We assume a uniform workload for each node in the cluster. In scenarios where the model fits entirely into a single node, this is trivial. However, when the model does not fit into a single node, this assumption becomes non-trivial. Indeed, several distributed training approaches strive to ensure that the workload is evenly distributed across the nodes, ~\cite{}, this cannot always be guaranteed. Consequently, emulating the behavior of only $\nbReal$ may be insufficient to predict the behavior of the entire cluster. To address this challenge, we propose classifying every node in the cluster based on the part of the model it holds, representing different stages in model parallelism. Subsequently, we emulate one node in each class. This approach enables us to infer the behavior by observing the collective behavior of each class. If there are $m$ stages in inter-node parallelism, we need to perform emulation $m$ times.

% \textcolor{red}{. For instance, if there are $k$ available nodes, we can distribute the emulation across multiple nodes, thereby reducing the number of iterations to $\frac{m}{k}$. This optimization helps streamline the emulation process and improve efficiency.}

% \subsection{Delay Computation Model}
% \textcolor{blue}{To emulate the delay induced by collective operations, we employ classical equations commonly used for analyzing collective operations \cite{thakur2005optimization}. Equation \ref{eqn:all-reduce} quantifies the delay caused by a ring allreduce operation in a cluster with $N$ nodes.}

% \begin{equation}
% \label{eqn:all-reduce}
%  T_{AllReduce}(N, M) = 2(N-1 ) * \alpha + 2(N-1)* M * \beta
% \end{equation}

% \textcolor{blue}{where $M$ represents the size of the message received from $\nbReal$, $\beta$ is defined as $\frac{1}{B}$, with $B$ denoting the link bandwidth. The value of $\alpha$ is determined through profiling on $\nbReal$. We note that other delay computation models and network simulators may offer different perspectives and nuances that could enhance our emulation of the collective operations. Exploring these alternatives in more detail is a direction we intend to pursue in future work.}

%\textcolor{green}{Justification of our approach: We would like to capture the effect of running the NCCL kernels on the real machines, so we decided to intercept the traffic outside to achieve a higher fidelity for the end-to-end behavior. Out of Memory Error: Currently model should fit in $\nbReal$. When it is not possible, we would need to produce atleast an instance of the model. Emulator node needs to have enough bandwidth to match the aggregate bandwidth of these nodes, to perform the emulation. We do not consider multiple emulator node at this point. ??}

\input{tab_coll}


\subsection{Proof-of-concept Implementation}

Our proof-of-concept implementation entails the development of an end-to-end system using the PyTorch DNN framework and NCCL as the collective communication library, chosen because of their popularity. 

Our implementation is able to run a two-node training using a distributed data-parallel strategy. In particular, we modify NCCL's instance in $\nbEnv$ to emulate the collective operations as per \cref{sec:design:uniform}. Moreover, in $\nbEnv$ we skip the \textsf{cudaKernelLaunch} completely so that no GPU computations are involved. We also modify the NCCL proxy so that it sends dummy data in compliance with the internal protocol so that the workload continues to run and $\nbReal$ is not aware of the emulation. In PyTorch, we mainly alter the \textsf{autogard} and \textsf{c10d} to implement the synchronization that previously relies on a CUDA kernel now compatible with the emulator.  We also remove computation in backward pass and model weight update in $\nbEnv$, given that those computations are redundant in emulation.

The whole system is about 2000 LoC in CUDA C++ and 50 LoC in Python, exclusive of experiments and tests.
%We evaluate the ability of the prototype emulator in the next section.
We plan to release \sys as open source.

% \banruo{do we need to talk about what has not yet to be done? i.e. topology detection, i.e. completely removing gpu involvement on emulator during the training?}
%There are also backends like Gloo or MPI, but since they are CPU-based, they do not suffer from the limited availability of high-end GPUs. However, our design for emulation is backend-independent.


% \textbf{c10d} is the abstraction for collective communication backend. The synchronization is done by monitoring cuda events associated with certain streams. Since our NCCL modifications bypass cuda kernel completely, the event is always marked complete even if the proxy threading is still transferring data. We modified c10d API make sure the API is semantically consistent with unmodified version by inserting barrier in at certain synchronization point.

% \textbf{autograd} we change \texttt{derivative.yaml} to remove computation in backward pass by returning an all zero tensor of desired output shape when possible. For matrix multiplication of $Y=AX$, where $A.shape=n*p, X.shape=p*m$, we return $Y=zeros(n*m)$

% \subsection{Outstanding features}

% The implementation of the \textbf{math model} is currently still pending. As an alternative, we use the simplest version of the fixed delay for this proof-of-concept version. However, since it is an independent module, we can easily extend it with sophisticated delay models. Also, the \textbf{topology detection} is currently not yet implemented, so strictly speaking we cannot run the emulation on a node without a GPU, even if we have already removed most of the computations. This also prevents us from running the experiment on multiple nodes.


==> sections/discussion.tex <==
We describe some pending technical challenges and our intuitions on how to tackle them.

\smartparagraph{Emulating many nodes.}
The proof-of-concept implementation only features a $2$-node cluster emulation. To emulate many nodes at once, we need to solve challenges including topology detection described in \ref{sec:design:init} and replace memory allocation interface since \sys's $\nbEnv$ has no GPUs.

% First, we intend to develop an interface with the PyTorch memory allocation function to prevent $\nbReal$ from encountering the Out of Memory (OOM) error during training initialization. %Second, we intend to develop the functionality that intercepts NCCL's topology discovery step. This will ensure that the training launch on $\nbReal$ keeps running under the impression that it is interacting with a full cluster. Second,


\smartparagraph{Communication model enhancements.}
For the proof-of-concept implementation, we have adopted a simple fixed delay model. For full implementation, we envision an interface for pluggable add-on components that can model delays at different levels of detail (i.e., tree topology) and capture system behaviors of large clusters (e.g., network congestion).

% For the proof-of-concept implementation, we have adopted a simple delay model from classical equations in the literature. However, we intend to integrate a more sophisticated approach into the full system implementation. In particular, we envision a flexible delay modelling component that is able to emulate/simulate collective operations at different levels of detail(i.e. tree topology) and efficiently capture peculiar system behaviours that occur in large clusters (e.g., congestion control).

\smartparagraph{Goodput prediction.}
The emulation is limited by the fact that we only emulate the \textbf{amount} of data transmitted over the network and not the actual \textbf{values} of the data.
This is enough to observe the time for each training iteration.
% However, this greatly complicates our ability to predict the accuracy of the model after training.
To support DNN training optimization techniques like lossy quantization and compression, \sys needs to also provide insights into the goodput of DNN models. One possible way is to run a proxy model~\cite{coleman2019selection} to produce data from a similar distribution.
This is a challenging yet meaningful direction that we would leave as future work.
% However, the question of how to make an accurate prediction of goodput under this paradigm is still an interesting direction for future work. 

% \subsection{Level Of Abstraction}
% We have chosen the collective communication layer as a suitable abstraction layer to mimic the behaviour of clusters and achieve a balance between complexity and accuracy. The reason for this is that emulation at the flow or packet level would be too fine-grained for training time estimation, which we want to perform, and would greatly increase the complexity of the implementation. On the other hand, we do not opt for a higher level of abstraction, such as nodes in computation graphs. This is because we currently only focus on emulating the ``outside world'' for a given node, and this level of abstraction is not suitable for this approach, nor does it allow us to capture the desired behaviour of the underlying network.

% %Being end-to-end allows us to support other strategies in an transparent way.

% \subsection{Fidelity}
% As discussed in previous sections, the fidelity of our results largely depends on following factors: ($1$) the end-to-end execution for node $N_0$ (and other node if we have a non-uniform setting) ($2$) the accuracy of delay computation model to calculate collective communication delay. 

% \subsection{Hardware Constraint}
% Since the emulation does send the data to node $N_0$ through network, we are unable directly to answer to hardware changes like ``what if bandwidth doubles'' due to lack of actual hardware to run the emulation. This might be helped with the "time dilation" technique that has been widely used in previous network emulation literature, but we will leave this as future work. \banruo{I am not sure whether time dilation can really helps, an alternative way is just to claim this is not the target of emulator, but that of simulators}



% \banruo{If we are considering ring all reduce in NCCL, more nodes mean more data. However, I believe the this increase would not burden the emulator. Because (1) there is a size cap for each message in NCCL, it will divide the original data into chunk with reasonable size and send it in multiple times. (2) For all reduce, $N_0$ is interacting with exactly 2 nodes(prev and next), so the emulator only need to emulate the data from that 2 nodes, regardless of the number of nodes.
% So the bandwidth on emulator won’t be a bottleneck But we need more time to run the all reduce, which means we need more time to run the emulation.}







==> sections/experiments.tex <==


We evaluate our prototype \sys implementation by ($1$) running microbenchmarks in NCCL level to see the pure performance of collective communication, ($2$) running an end-to-end system in PyTorch to see the accuracy of emulation, as well as measuring CPU utilization to evaluate the overheads of \sys. We also demonstrate ($3$) an application scenario of \sys by performing a ``what-if'' analysis with latency variations.

\vspace{0.1in}
\smartparagraph{Testbed.} Our test environment consists of two nodes, each equipped with two 8-core Intel Xeon Silver 4112 CPUs running at 2.60 GHz, 512 GB RAM and is fitted with a 100 GbE Mellanox ConnectX-5 NIC. In addition, each node contains two NVIDIA V100 GPUs, although only one is used during evaluation. Each node runs Ubuntu 22.04 (Linux kernel 5.15.0), CUDA 12.2, PyTorch 2.2.0a0 and NCCL 2.19.4.

If not otherwise stated, we call the two nodes $\nbReal=\{N_0\}$ and $\mathcal{E} = \{N_{emu}\}$. $N_0$ always runs the unmodified code. $N_{emu}$ is configured to run either \sys's modified code(as emulator), or unmodified modified code (as a baseline).

\subsection{Microbenchmark}

\smartparagraph{Setup.} First we assess \sys's capability to emulate collective communication operations. We devise the benchmark by generating input data tensors of different sizes on GPU and issuing two-node collective operations. We test \textsf{ncclAllreduce} and \textsf{ncclAllgather}. After warm-up, we measure the time taken over at least 100 repetitions for each call on $N_{emu}$ and report the average. $N_0$ always runs unmodified code. We compare the result when $N_{emu}$ is running unmodified NCCL (baseline) and \sys's NCCL (emulator).

% \textbf{Setup}.We run a program that constantly sends a sufficiently large number of collective operations. This scenario simulates the use case in PyTorch. We run the collective operation on two nodes, $N_0$ and $N_{emu}$, $N_0$ always executes unmodified NCCL, and $N_{emu}$ executes \sys or unmodified NCCL (as a base). We record the average time for each call after warming up to $N_{emu}$ and compare the result of \sys and baseline.


% \begin{figure}[htb]
% \centering { 
% \includesvg[width=\linewidth]{images/coll.svg}
%  \caption{The relative time($\frac{t_{Neurona}}{t_{baseline}}$) for Allreduce and Allgather.}
%   \vspace{4mm}
%   \label{fig:coll}
%   }
% \end{figure}

\smartparagraph{Results.} \cref{tab:coll} shows that \sys only incurs at most 4\% overhead; we attribute this to the mutex lock on the controller and bitmap bookkeeping. The overhead diminishes as the size increases; when the size is greater than 2MB, the gap is no more than 1\%. Since most data parallel implementations use buckets to batch all-reduce calls to a larger size (e.g., 25MB in NVIDIA APEX ~\cite{nvidiaapex}), we believe this NCCL-level overhead of \sys is acceptable. 
% \begin{table}[h!]
% \centering
% \begin{tabular}{||c c c c c||} 
%  \hline
%  Model & Time-Emu & Time-Base & CPU-Emu & CPU-base \\ [0.5ex] 
%  \hline\hline
%  BERT & 629 $\pm$ 3.0  & 628$\pm$1.1 & 1.21 & 1.45  \\ 
%  ResNet152 & 1061$\pm$19.8 & 1063$\pm$16.3  &1.23 &1.59 \\
%  DeepLight & 727$\pm$15.0  & 726$\pm$ 13.8  & 0.80 & 0.81   \\[1ex] 
%  \hline
% \end{tabular}
% \caption{The result of the end-to-end system. `Emu' and `Base' stand for emulator enabled and baseline, respectively. `Time' stands for the training time and is measured in ms; and `CPU' stands for the CPU usage during training and is measured in the number of cores. All data is collected by the emulator node.}
% \label{table:e2e_results}
% \end{table}

\subsection{End-to-end Training Emulation}

\smartparagraph{Setup.} To evaluate \sys's ability to accurately emulate end-to-end DNN training, we conducted experiments using three real-world DNN models, including computer vision, natural language processing and recommendation systems. The models details are listed in \cref{table:model}. We use PyTorch's \textsf{DistributedDataParallel} module for data parallelism. $N_0$ runs unmodified PyTorch; $N_{emu}$ runs \sys's PyTorch as emulator and unmodified PyTorch as baseline. 

We measure the metrics and report the average after warm-up. We report training time per iteration for BERT and ResNet; we report training time per epoch for DeepLight because it involves model pruning and has variance in between iterations. We also measure the CPU usage in \sys to illustrate the overhead of the emulation.
%We \textsf{mpstat} on a consecutive 10 five-second intervals after warmup.
% We observed that the number of training samples processed per unit time stabilizes after about $100$ iterations. Therefore, we excluded the first $100$ iterations from our performance analysis to minimize noise and focused on the subsequent $200$ iterations to obtain consistent and accurate results. The primary performance metric reported for ResNet and BERT was the difference between the observed training time per iteration observed from the actual system run and those predicted by the emulator. For DeepLight, we have specified the training time per epoch. The difference in the choice of metric is due to the unique properties of the DeepLight model, which include trimming, resulting in different iteration lengths.

\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||l r r r||} 
 \hline
 Model & Task & Dataset & Size \\ [0.5ex] 
 \hline
 BERT ~\cite{devlin2018bert}& Question Answer  & SQuAD ~\cite{rajpurkar2018squad} &   1.28GB \\ 
 ResNet152 ~\cite{he2016resnet} & Image Classify & ImageNet-1K ~\cite{russakovsky2015imagenet}& 230MB \\
 DeepLight ~\cite{deng2021deeplight} & Click Predict &  Criteo 1TB ~\cite{Criteo1t}  & 2.26GB   \\[0.5ex] 
 \hline
\end{tabular}
}
\caption{Characteristics of benchmark DDN models, size represents the total parameter size of a model.}
\label{table:model}

\begin{tabular}{||l r r r r||} 
 \hline
 Model & Time-E & Time-B & CPU-E & CPU-B \\ [0.5ex] 
 \hline
 BERT & 629 $\pm$ 3.0  & 628$\pm$1.1 & 12.93\% & 14.25\%  \\ 
 ResNet152 & 1061$\pm$19.8 & 1063$\pm$16.3  &12.68\% &12.95\% \\
 DeepLight & 727$\pm$15.0  & 726$\pm$ 13.8  & 7.52\% & 7.75\%   \\[0.5ex] 
 \hline
\end{tabular}

\caption{End-to-end workload comparison. `E' and `B' stand for emulator-enabled (\sys) and the baseline, respectively. `Time' stands for the training times in milliseconds; and `CPU' stands for the percentage of CPU usage in a node.}
\label{table:e2e_results}
\end{table}

\smartparagraph{Results.} As shown in \cref{table:e2e_results}, \sys is quite accurate in a two-node environment training with data parallelism, with error less than 1\%. 
For CPU usage, it actually drops a little bit in all scenario. We attribute that to: ($1$) the efficient and lightweight implementation of \sys, which keeps the overhead generally low; ($2$) the removal of computation in backward pass, which eliminates a lot of memory allocation and data movements. So the net effect is a drop in CPU usage. This is promising in terms of the potential scalability of \sys.

\subsection{What-if Analysis: Latency}

\smartparagraph{Setup.} In this experiment, $N_0$ runs unmodified code and $N_{emu}$ runs \sys. We inject additional delay in each all-reduce call in $N_{emu}$ and train a BERT model. We measure the emulated training time per iteration for each delay.

\smartparagraph{Results.} As \cref{fig:delay} shows, the iteration time increases linearly with the delay larger than 2 milliseconds. However, when the delay is small, the overheads reflected in the end-to-end performance does not grow linearly. We consider this ``smooth slope'' as a result of the computation-communication overlap during the training. The delay injected in each all-reduce call is partly shadowed by the async computation in the backward pass. Such observation implies a possible space of improvement in the training, as there is a "2ms" space for more communication to happen. This is an example of the kind of insights that can be obtained from using \sys.

\begin{figure}[t!]
\centering 
\includegraphics[width=0.975\linewidth]{images/delay_vs_average.pdf}
 \caption{The end-to-end training time per iteration in BERT model (ms) vs the additional delay injected in every all reduce call (ms). Error bar is plotted in black.}
  \vspace{4mm}
  \label{fig:delay}
\end{figure}

% Our experiments aim to answer the following questions

% \begin{itemize}
%     \item Does the prototype show the technical possibility of emulator depicted in design section?
%     \item Are the results provided by the emulation accurate?
%     \item Does emulation reduce cost for testing ddl strategy?
%     \item Can emulation answer what-if questions?
% \end{itemize}

% \subsection{Accuracy}

% \todo{
%      A curve of e2e per operation latency v.s. throughput. The e2e latency is obtained by inject artificial delay + inherent latency. By changing the injected delay, we measure the throughput and get the curve.
    
%      Run the actual model without an emulator, measure the latency and throughput, and see if the actual throughput matches our emulated throughput. (The point is close enough to the curve.)
% }

% \subsection{What-if Question}




==> sections/idea.tex <==
We provide an emulator for distributed training, which effectively emulates the outside environment for a single node, making it believe that it is running a distributed training job, where the rest of comm is actually emulated.

We modify the underlying collective communication library(i.e. Nvidia NCCL) to allow us return arbitrary amount of data and inject artificial delay during the training.

\subsection*{Arguments}

Our design is good(bad) because:

\begin{itemize}
  \item Reduce cost
    \begin{itemize}
      \item Mordern model traning requires thousands of GPUs traning many hours or days. Our emulator only requires a single node and its GPUs. 
      \item \banruo{However, our emulation runs exactly the same amount of time, which is slower than simulation. But we can argue that we only need to run a single epoch.}
    \end{itemize}
  \item Adapt to new strategy
    \begin{itemize}
        \item Unlike previous simulator that implement various training strategies within the simulator, our emulation is done by intercepting the collective communication primitives. So, we automatically support new strategies as long as they still use collective communication.

    \end{itemize}
  \item More Accurate
    \begin{itemize}
        \item Since we actually run the training on a node, it is intuitively more accurate than analytical simulation. Because the real system implementation are taken into account.\banruo{However, one might argue simulator can also use profiling results}
    \end{itemize}
\end{itemize}

\subsection*{Experiments}

Suppose we have our emulator, our experiments should include

\subsection{what-if}
Our emulation can provide answers to questions like "what if the bandwidth doubles(no current hardware available)

\begin{itemize}
    \item A curve of e2e per operation latency v.s. throughput. The e2e latency is obtained by inject artificial delay + inherent latency. By changing the injected delay, we measure the throughput and get the curve.
    \item Run the actual model without an emulator, measure the latency and throughput, and see if the actual throughput matches our emulated throughput. (The point is close enough to the curve.)
    \item Then we claim that our emulator can be used to study the behaviour when the hardware becomes more advanced (lower latency). How will the throughput change, which is the part of the curve whose x is smaller than the calculated real latency?
\end{itemize}
\subsection{accuracy}
 Compare predicted latency on various model, this overlaps with "what-if".w

\subsection{support new strategy}
Show LoC that need to implement FSDP in simulator?



==> sections/introduction.tex <==

Modern DNN training clusters are remarkable engineering feats that more closely resemble high-performance specialized computing environments -- and the large costs that these entail -- than their mainstream counterparts in commodity cloud computing datacenters.
Optimizing resource utilization and overall efficiency is paramount to maximizing the performance of training workloads and minimizing associated costs.
Therefore, it is highly desirable to explore the large space of potential design considerations, performance optimizations and configuration tunings, and ideally to do so without incurring time, energy, and monetary costs of profiling training workloads at scale on actual hardware.

Conducting in-depth ``what if'' analyses is essential to making informed decisions and beneficial for a variety of scenarios. For instance, a ML engineer may want to explore for a given model the impact of a particular parallelization strategy\footnote{Possible strategies include data parallelism~\cite{xing2015petuum}, tensor parallelism~\cite{shoeybi2020megatronlm}, pipeline parallelism~\cite{huang2019gpipe}, fully sharded data parallelism~\cite{zhao2023pytorch} among others.} on the training time and resource utilization.
But it is not practical to profile the training workload on thousands of HW accelerators (GPUs, TPUs, etc.) for each possible strategy and different configurations.
Similarly, a researcher may want to quantify the benefits \emph{at scale} of a new optimization technique to improve LLM training efficiency. Also in this case, it is hardly feasible to run systematic experiments on a large cluster for each possible configuration.

Recent work has shown the potential of simulation and analytical methods to gain insights about DNN training behavior~\cite{rashidi2020astra, rashidi2022themis, esposito2022dts, ardalani2022deepflow, won2023astra, bang2023vtrain}. However, these approaches suffer from at least one of three limitations:
\begin{inparaenum}[1)]
\item they require significant effort to transform the actual workloads into an input model for the simulator,
\item they require explicit models of parallelization strategies and incorporating new ones entails non-trivial development of new simulation models, and,
\item the fidelity of their results is limited by how faithful the underlying analytical models of compute and communication are, which are notoriously difficult to get right at scale~\cite{mittal2018rocerdma}.
\end{inparaenum}

\begin{figure}[t!]
    \centering
    \includegraphics[trim={0 1.2cm 0 0},clip, width=0.975\linewidth]{images/machine_view.pdf}

\caption{A training job running in a 4-node cluster (left) is emulated by executing a single real node ($N_0$) wrapped by \sys, which emulates the environment (right).}
    \label{fig:neuornabox}
\end{figure}

This work pioneers and advocates the use of emulation to aid in the analysis and experimentation of distributed DNN training workloads.
What we mean by emulation is illustrated in \cref{fig:neuornabox}. In a nutshell, we propose to isolate a node subset (denoted as $\nbReal$) of a distributed training job and emulate the networked execution environment (denoted as $\nbEnv$) from the perspective of the nodes in $\nbReal$.
We elect to view the network as a natural boundary between the real and emulated environments since communication between nodes in distributed training jobs typically occurs through a collective communication library (e.g., NCCL~\cite{nccl}) that both isolates the training scripts from dealing with all the unnecessary details of the underlying network and demarcates clear points for inter-process synchronization.
We refer to our approach as \sys.

Notably, in this approach, the nodes in $\nbReal$ run unmodified training scripts, DNN frameworks and libraries. In particular, the communication is handled by the actual collective communication library over the network fabric.
Meanwhile, the emulation environment $\nbEnv$ executes on dedicated hardware resources. The requirements for the emulation environment are modest: it doesn't require HW accelerators, it can run on a single CPU-based node, and it requires network bandwidth to match the available aggregate bandwidth of nodes in $\nbReal$.

The key benefit of this approach is that it allows us to faithfully execute on real hardware a portion of the training workload, which executes without overheads from instrumentation (since there is none) nor profiling $\nbReal$ in controlled conditions.
Therefore, we can observe the actual behavior of the training job, including the HW utilization metrics and collective communication patterns that are critical in analyzing the performance of distributed training workloads.

We wish to stress that our objective is to enable performance analysis and optimization of distributed training workloads. Implications on model quality are out of scope.

Thus, in this work, we initiate the study of these core research questions:
\begin{inparaenum}[1)]
    \item \emph{What aspects of the workload must $\nbEnv$ emulate?}
    \item \emph{How can this approach maintain high fidelity while retaining wide applicability?}
\end{inparaenum}

With this short paper, we aim to provide an initial exploration of the feasibility and potential of this approach, and to solicit feedback from the community on the soundness of our approach and the prospects for future research.


% Why is this beneficial?
% Why this is challenging?
% Why this can be trusted?

%The groundbreaking achievements recorded by Deep Neural Networks (DNNs) in recent years are significantly propelled by the robust compute, memory, and network capabilities offered by modern data centers and dedicated AI clusters. However, a significant amount of the compute resources in these clusters remain largely unused, with utilization rates hovering around 30–45\% when training large models~\cite{shoeybi2020megatronlm, wang2023zero++}. 
%Efficient system configuration is essential to optimizing cluster utilization and addressing the escalating costs of training large Deep Neural Network (DNN) models. However, the prohibitive time and cost implications of exploring different configurations on real hardware emphasize the need for a fast, cost-effective, and high-fidelity approach to testing cluster configurations prior to deployment for DNN training. Such an approach would enable system designers to perform in-depth ``what if'' analyses and experiment with different configurations and scenarios. This will ensure that DNN training system design decisions are quick, informed, and cost-effective.

%Recent research has shown the potential of analytical methods to capture DNN training behavior without the need to run the actual workload on real hardware~\cite{won2023astra}. This development has led to many research efforts to develop analytical simulators for the optimization of DNN training~\cite{rashidi2020astra, rashidi2022themis, esposito2022dts, ardalani2022deepflow, won2023astra}. However, these simulators suffer from one or more of three limitations: ($1$) they require significant technical effort to convert the model workloads into the simulator's input format, ($2$) they lack the agility to adapt to new distributed training approaches; or ($3$) they estimate training time only based on the execution time profiles of the compute accelerators and do not take the collective communication overhead into account. 

% Efficient training and cluster configurations can significantly reduce the waste of very scarce compute resources and maximize the performance of DNN training. However, optimizing the performance of AI clusters depends on a multi-faceted approach that involves compute, memory, and network optimizations. The associated intricacies, such as model (hyper)parameters, workload distribution, job scheduler logic, partitioning strategy, topology, and hardware specifications, form a complex landscape. Testing all possible combinations of the system/workload design options and their associated performance implications is unrealistic, as that will be prohibitively expensive and time-consuming. To navigate the complexities of ML system design and overcome the prohibitive time and cost implications of testing each of the design decisions on actual clusters, a simulator or emulator platform emerges as an indispensable tool. Such a platform would enable organizations to perform in-depth ``what if'' analyses and experiment with different configurations and scenarios. By providing a controlled environment for exploratory analysis, a simulator or emulator ensures that DNN training system design decisions are quick, informed, and cost-effective.

% \smartparagraph{Limitation of existing simulation-based approaches}. Recent research has shown the potential of analytical methods to capture training behavior without the need to run the actual workload on real hardware~\cite{won2023astra}. This development has led to many research efforts to develop analytical simulators for the optimization of DNN training~\cite{rashidi2020astra, rashidi2022themis, esposito2022dts, ardalani2022deepflow, won2023astra}. However, these simulators suffer from one or more of three limitations: ($1$) they require significant technical effort to convert the model workloads into the simulator's input format, ($2$) they lack the agility to adapt to new distributed training approaches; or ($3$) they are not available to the public. %\banruo{($4$)Their analytical approach also cannot faithfully simulate hardware features, i.e. infiniband, but I have no evidence that such neglect will result in significantly less accurate result}

% \begin{figure}[t!]
%     \centering
%     {
%   \includegraphics[width=0.975\linewidth]{images/machine_view.pdf}
%   }
%   \caption{An example to illustrate a cluster with four nodes. Left side represents is the normal setting, where right side we use \sys to emulate the outside world for node $A$, the data transfer within the emulation is effectively omitted.}
% \label{fig:machine_view}
% \end{figure}

% \smartparagraph{This research}. This work proposes \sys: a novel emulator-based approach that mitigates the aforementioned limitations of the existing approaches. Specifically, \sys is based on the following observations: First, all distributed training jobs are launched from a single machine node (say ``Node 0'' or $N_0$ for short), which is then responsible for processing the system configuration, detecting the available hardware resources, and launching the training job. Second, for nearly all distributed training paradigms, the workload distribution policy strives to achieve a balance, such that collective communication can commence around the same time across all workers~\cite{shoeybi2020megatronlm, li2023colossal, rajbhandari2020zero}. This makes the behavior of all nodes almost identical. What varies, however, is the collective communication operations that are employed during gradient/weight synchronization. The completion time of these collective operations is influenced by the type of operation, network topology, bandwidth, and other system configuration decisions. And lastly, to achieve accurate predictions regarding the performance of a distributed training workload within a specified cluster configuration, it suffices to emulate the behavior of $N_0$, and the underlying collective communication operations that are defined for the adopted distributed training strategy.


% Based on the above observations, we propose \sys, which is able to launch distributed training tasks with any leading ML framework, such as PyTorch~\cite{paszke2019pytorch}, on any node $N_0$ and generate performance metrics relevant to the given training cluster configuration by emulating the rest of the cluster. \sys can faithfully emulate the system behavior, focusing on the end-to-end behavior for a representative segment of the training job and the associated collective communication operations. Figure~\ref{fig:neuornabox} illustrates a high-level representation of \sys. On the left side of the picture is a depiction of an actual training cluster with four interconnected nodes: $N_0$, $N_1$, $N_2$, and $N_3$. To emulate this cluster, \sys launches the DNN training on 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.975\linewidth]{images/Neurona}

% \caption{An example to illustrate a cluster with four nodes. The left side represents the normal setting, and on the right side, we use \sys to emulate the rest of the cluster from $N_0$'s perspective.}
%     \label{fig:neuornabox}
% \end{figure}

%The proposed emulator can potentially mimic a real cluster environment by seamlessly interacting with the collective communication library on $N_0$. This approach offers a unique advantage by allowing comprehensive investigations of various cluster behaviors, including responses to dynamic events such as bandwidth changes, topology changes, distributed training strategies, collective communication algorithms, gradient aggregation window adjustments, data compression, and tensor fusion batch size alterations.

% \textbf{Contribution}. % This owrk pioneers and advocates the use of emulation to analyze distributed DNN training, focusing on the critical bottleneck of low-level collective communication patterns. While emulation has proven successful in networking, its application to distributed training presents unique challenges. In contrast to well-defined network protocols, complex and evolving parallelization strategies are characteristic of distributed deep learning training. To navigate these intricacies, we decompose distributed training into emulatable components and focus on the collective communication component to evaluate cluster performance.
% To the best of our knowledge, this work represents the first attempt to study DNN training time by running a portion of the training on a real node and emulating the rest of the cluster. In addition, our work differs from the others in the following key aspects: 

% \begin{itemize}
%     \item \textbf{User-Friendliness:} To the best of our knowledge, this is the first DNN training emulator that can take a training script directly as workload input without requiring significant technical effort (e.g., profiling or gathering execution trace).

%      \item \textbf{Flexibility:} \sys ensures that the emulator can support any parallelization strategy, including those yet to be developed as of today, provided that these strategies employ the well known collective communication operations in distributed training.

%     \item \textbf{Proof-of-concept:} We also provide a proof of concept implementation of \sys. Extensive experiments demonstrate its ability to accurately predict execution time across various workloads.
    
% \end{itemize}

%\textbf{Paper organization}. The rest of this paper is structured as follows. Section~\ref{Sec:background} provides some relevant contexts that are essential for a seamless understanding of our contributions. Section~\ref{sec:design} elaborates on the design principles, workflow, and the delineation of the emulator components. Following this, Section~\ref{sec:implementation} elucidates the implementation process, while Section~\ref{sec:experiments} presents experimental results demonstrating the efficacy of the emulator in accurately capturing the behavior of distributed training systems. In Section~\ref{sec:related_work}, we discuss some related works, and finally, Section~\ref{sec:conclusion} concludes the paper with some future research direction.

==> sections/related_work.tex <==
\smartparagraph{DDL simulation.} A number of simulators have been developed to study the behavior of DNN clusters, including DeepFlow\cite{ardalani2022deepflow}, Astra-sim~\cite{rashidi2020astra,won2023astra}, vTrain~\cite{bang2023vtrain} and several others~\cite{rashidi2022themis, esposito2022dts, stanic2023languini, hestness2017deep}. These simulators use analytical methods combined with profiling results to make predictions, suffering from limitations mentioned in \cref{sec:introduction}.

% These tools have proven useful to the research community but suffer from two major limitations that our approach attempts to address. First, the parallelization scheme to be simulated must be explicitly supported, and in some cases, the number of supported schemes is limited. Moreover, they are not easy to use and require special operations to generate the inputs (e.g., creating execution graphs or system logs). In contrast, our proposed emulator can mirror the behavior of any parallelization strategy and use the Pytorch model implementation as input without requiring any input generation.

% Some other works~\cite {stanic2023languini, hestness2017deep} use some linear models to estimate the training time of DNNs, based on the available compute resources in FLOPs.A limitation of this approach is that the assumption about the available FLOPs does not take into account different system characteristics and configurations (e.g., bandwidth, topology, distributed training strategy, etc.) that could affect the available compute resources.

% The vTrain simulator~\cite{bang2023vtrain} is the most comparable work to our proposal. It focuses on estimating the training time of Large Language Models (LLMs)~\cite{devlin-etal-2019-bert, brown2020language} using a profiling-based approach. While vTrain and our proposal have similarities in that they only use the model description and configuration as input, they differ significantly in their underlying approaches and objectives. First, vTrain is specifically tailored to LLMs, whereas our emulator is designed to accommodate any DNN model. Second, vTrain's training time estimates are mainly based on the execution time profiles of the GPU kernel operations associated with each LLM layer. In contrast, our emulator incorporates collective communication time modeling.

%\noindent \textbf{Distributed system emulation}.

\smartparagraph{Network emulation.} Emulation has been widely adopted in networking research~\cite{modelnet,mininet}. MimicNet~\cite{zhang2021mimicnet} is a machine learning based network emulator. It exercises a similar idea by dividing the datacenter into an ``observable'' cluster ($\nbReal$ in our work) and a blackbox ($\mathcal{E}$ in our work) and it applies a machine learning model to fit it. However, MimicNet focuses on how to train a model to better approximate the datacenter network at scale, whereas our work focuses on emulating end-to-end DNN training behaviors. %and aims to provide an emulation abstraction and interface that is flexible and user-friendly.

\smartparagraph{Goodput prediction.}
Currently, \sys only sends \textit{dummy} data to $\mathcal{N}$ during emulation since it only predicts the completion time for each training iteration. However, lossy training optimization techniques like compression and quantization ~\cite{wang2023zero++, lin2017gradientcompression} require goodput (accuracy) to be taken into account. To support that, \sys needs to communicate \textit{meaningful} data to $\mathcal{N}$ without incurring much overhead. One possible solution is to use a proxy model~\cite{coleman2019selection} that generates data with a similar distribution to the dataset and intermediate results.

%To emulate DNN training optimization techniques such as lossy quantization and compression~\cite{wang2023zero++, lin2017gradientcompression}, it is required that not only the \textit{amount} of data be emulated but also the \textit{value} of the data. The current implementation of \sys only predicts the iteration time by sending \textbf{dummy} data through the network. It must send \textit{meaningful} data to effectively support these lossy strategies. One possible approach is to use a proxy model~\cite{coleman2019selection} that generates data with a similar distribution to the original training set. 


